Query Recovery from Easy to Hard: Jigsaw Attack against SSE

Searchable symmetric encryption schemes often unintentionally disclose certain sensitive information, such as access, volume, and search patterns. Attackers can exploit such leakages and other available knowledge related to the user's database to recover queries. We find that the effectiveness of query recovery attacks depends on the volume/frequency distribution of keywords. Queries containing keywords with high volumes/frequencies are more susceptible to recovery, even when countermeasures are implemented. Attackers can also effectively leverage these ``special'' queries to recover all others. By exploiting the above finding, we propose a Jigsaw attack that begins by accurately identifying and recovering those distinctive queries. Leveraging the volume, frequency, and co-occurrence information, our attack achieves $90\%$ accuracy in three tested datasets, which is comparable to previous attacks (Oya et al., USENIX' 22 and Damie et al., USENIX' 21). With the same runtime, our attack demonstrates an advantage over the attack proposed by Oya et al (approximately $15\%$ more accuracy when the keyword universe size is 15k). Furthermore, our proposed attack outperforms existing attacks against widely studied countermeasures, achieving roughly $60\%$ and $85\%$ accuracy against the padding and the obfuscation, respectively. In this context, with a large keyword universe ($\geq$3k), it surpasses current state-of-the-art attacks by more than $20\%$.

==> figures_against_CGPR.tex <==

\begin{figure}[!h]
	\centering
	\subfigure[Enron]
	{
 \label{fig:padding_CGPR_enron}
		\begin{minipage}{.45\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Reenron_padding_1000.pdf}
		\end{minipage}
	}
	\subfigure[Lucene]
	{
 \label{fig:padding_CGPR_lucene}
		\begin{minipage}{.45\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Relucene_padding_1000.pdf}
		\end{minipage}
	}
	\caption{Comparison with RSA and IHOP attacks against the padding in CGPR\cite{cash2015leakage} in Enron and Lucene.}
	\label{fig:against_CGPR_enron_lucene}
\end{figure}


\begin{figure*}[!h]
	\centering
	\subfigure[$|W|=1000$]
	{
 \label{fig:padding_CGPR_wiki_1000}
		\begin{minipage}{.30\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Rewiki_padding_1000.pdf}
		\end{minipage}
	}
	\subfigure[$|W|=3000$]
	{
 \label{fig:padding_CGPR_wiki_3000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_padding_3000.pdf}
		\end{minipage}
	}
        \subfigure[$|W|=5000$]
	{
 \label{fig:padding_CGPR_wiki_5000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_padding_5000.pdf}
		\end{minipage}
	}
	\caption{\color{blue}Comparison with RSA and IHOP attacks against the padding in CGPR\cite{cash2015leakage} in Wikipedia.}
	\label{fig:against_CGPR_wiki}
\end{figure*}


==> figures_against_cluster_based_padding.tex <==
\begin{figure}[!h]
	\centering
	\subfigure[Enron]
	{
 \label{fig:padding_cluster_enron}
		\begin{minipage}{.45\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Reenron_padding_cluster_1000.pdf}
		\end{minipage}
	}
	\subfigure[Lucene]
	{
 \label{fig:padding_cluster_lucene}
		\begin{minipage}{.45\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Relucene_padding_cluster_1000.pdf}
		\end{minipage}
	}
	\caption{{\color{blue}Comparison with RSA and IHOP attacks against the cluster-based padding\cite{DBLP:journals/corr/shielddb} in Enron and Lucene.}}
	\label{fig:against_padding_cluster_enron_lucene}
\end{figure}

\begin{figure*}[!h]
	\centering
	\subfigure[$|W|=1000$]
	{
 \label{fig:padding_cluster_wiki_1000}
		\begin{minipage}{.30\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Rewiki_padding_cluster_1000.pdf}
		\end{minipage}
	}
	\subfigure[$|W|=3000$]
	{
 \label{fig:padding_cluster_wiki_3000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_padding_cluster_3000.pdf}
		\end{minipage}
	}
        \subfigure[$|W|=5000$]
	{
 \label{fig:padding_cluster_wiki_5000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_padding_cluster_5000.pdf}
		\end{minipage}
	}
	\caption{{\color{blue}Comparison with RSA and IHOP attacks against the cluster-based padding\cite{DBLP:journals/corr/shielddb} in Wikipedia.}}
	\label{fig:against_padding_cluster_wiki}
\end{figure*}

==> figures_against_obfuscation.tex <==
\begin{figure}[!h]
	\centering
	\subfigure[Enron]
	{
 \label{fig:obfuscation_enron}
		\begin{minipage}{.45\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Reenron_obfuscation_1000.pdf}
		\end{minipage}
	}
	\subfigure[Lucene]
	{
 \label{fig:obfuscation_lucene}
		\begin{minipage}{.45\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Relucene_obfuscation_1000.pdf}
		\end{minipage}
	}
	\caption{{\color{blue}Comparison with RSA and IHOP attacks against the obfuscation in CLRZ\cite{DBLP:conf/infocom/ChenLRZ18} in Enron and Lucene.}}
	\label{fig:against_obfuscation_enron_lucene}
\end{figure}

\begin{figure*}[!h]
	\centering
	\subfigure[$|W|=1000$]
	{
 \label{fig:obfuscation_wiki_1000}
		\begin{minipage}{.30\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Rewiki_obfuscation_1000.pdf}
		\end{minipage}
	}
	\subfigure[$|W|=3000$]
	{
 \label{fig:obfuscation_wiki_3000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_obfuscation_3000.pdf}
		\end{minipage}
	}
        \subfigure[$|W|=5000$]
	{
 \label{fig:obfuscation_wiki_5000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_obfuscation_5000.pdf}
		\end{minipage}
	}
	\caption{{\color{blue}Comparison with RSA and IHOP attacks against the obfuscation in CLRZ\cite{DBLP:conf/infocom/ChenLRZ18} in Wikipedia.}}
	\label{fig:against_obfuscation_wiki}
\end{figure*}

% \begin{figure*}[!h]
% 	\centering
% 	\subfigure[Enron]
% 	{
%  \label{fig:obfuscation_enron}
% 		\begin{minipage}{.30\linewidth}
% 			\centering
%                 \includegraphics[width=\linewidth]{pic/test_IHOP_with_alpha/enron_obfuscation_1000.pdf}
% 		\end{minipage}
% 	}
% 	\subfigure[Lucene]
% 	{
%  \label{fig:obfuscation_lucene}
% 		\begin{minipage}{.30\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_IHOP_with_alpha/lucene_obfuscation_1000.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[Wikipedia]
% 	{
%  \label{fig:obfuscation_wiki}
% 		\begin{minipage}{.30\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_IHOP_with_alpha/wiki_obfuscation_3000.pdf}
% 		\end{minipage}
% 	}
% 	\caption{{\color{blue}IHOP with different $\alpha$.}}
% 	\label{fig:IHOP_alpha}
% \end{figure*}


==> figures_against_padding_seal.tex <==
\begin{figure}[!h]
	\centering
	\subfigure[Enron]
	{
 \label{fig:padding_seal_enron}
		\begin{minipage}{.45\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Reenron_padding_seal_1000.pdf}
		\end{minipage}
	}
	\subfigure[Lucene]
	{
 \label{fig:padding_seal_lucene}
		\begin{minipage}{.45\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Relucene_padding_seal_1000.pdf}
		\end{minipage}
	}
	\caption{{\color{blue}Comparison with RSA and IHOP attacks against the padding in SEAL\cite{DBLP:conf/uss/DemertzisPPS20} in Enron and Lucene.}}
	\label{fig:against_padding_seal_enron_lucene}
\end{figure}

\begin{figure*}[!h]
	\centering
	\subfigure[$|W|=1000$]
	{
 \label{fig:padding_seal_wiki_1000}
		\begin{minipage}{.30\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/against_countermeasures/Rewiki_padding_seal_1000.pdf}
		\end{minipage}
	}
	\subfigure[$|W|=3000$]
	{
 \label{fig:padding_seal_wiki_3000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_padding_seal_3000.pdf}
		\end{minipage}
	}
        \subfigure[$|W|=5000$]
	{
 \label{fig:padding_seal_wiki_5000}
		\begin{minipage}{.30\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/against_countermeasures/Rewiki_padding_seal_5000.pdf}
		\end{minipage}
	}
	\caption{{\color{blue}Comparison with RSA and IHOP attacks against the padding in SEAL\cite{DBLP:conf/uss/DemertzisPPS20} in Wikipedia.}}
	\label{fig:against_padding_seal_wiki}
\end{figure*}



% \begin{figure*}[!h]
% 	\centering
 
% 	\subfigure[Enron]
% 	{
%  \label{fig:padding_SEAL_enron}
% 		\begin{minipage}{.30\linewidth}
% 			\centering
%                 \includegraphics[width=\linewidth]
%                 {pic/against_countermeasures/enron_padding_seal_1000.pdf}
% 		\end{minipage}
% 	}
% 	\subfigure[Lucene]
% 	{
%  \label{fig:padding_SEAL_lucene}
% 		\begin{minipage}{.30\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/against_countermeasures/lucene_padding_seal_1000.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[Wikipedia]
% 	{
%  \label{fig:padding_SEAL_wiki}
% 		\begin{minipage}{.30\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/against_countermeasures/wiki_padding_seal_1000.pdf}
% 		\end{minipage}
% 	}
 
% 	\caption{Comparison with RSA and IHOP attacks against the padding in SEAL\cite{DBLP:conf/uss/DemertzisPPS20}.}
% 	\label{fig:against_the_padding_in_seal}
% \end{figure*}


==> figures_in_experiment_of_our_attack.tex <==
\begin{figure*}[!t]
	\centering
	
	\subfigure[HVHF]
	{
 \label{HVHF_3D_Enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/HVHF_3D.pdf}
		\end{minipage}
	}
	\subfigure[HVLF]
	{
 \label{HVLF_3D_Enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/HVLF_3D.pdf}
		\end{minipage}
	}
        \subfigure[LVHF]
	{
 \label{LVHF_3D_Enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/LVHF_3D.pdf}
		\end{minipage}
	}
        \subfigure[LVLF]
	{
 \label{LVLF_3D_Enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/LVLF_3D.pdf}
		\end{minipage}
	}
	
	
	\subfigure[HVHF]
	{
 \label{HVHF_3D_Lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/HVHF_3D.pdf}
		\end{minipage}
	}
	\subfigure[HVLF]
	{
 \label{HVLF_3D_Lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/HVLF_3D.pdf}
		\end{minipage}
	}
        \subfigure[LVHF]
	{
 \label{LVHF_3D_Lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/LVHF_3D.pdf}
		\end{minipage}
	}
        \subfigure[LVLF]
	{
 \label{LVLF_3D_Lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/LVLF_3D.pdf}
		\end{minipage}
	}
	
	
	\subfigure[HVHF]
	{
 \label{HVHF_3D_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/HVHF_3D.pdf}
		\end{minipage}
	}
	\subfigure[HVLF]
	{
 \label{HVLF_3D_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/HVLF_3D.pdf}
		\end{minipage}
	}
        \subfigure[LVHF]
	{
 \label{LVHF_3D_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/LVHF_3D.pdf}
		\end{minipage}
	}
        \subfigure[LVLF]
	{
 \label{LVLF_3D_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/LVLF_3D.pdf}
		\end{minipage}
	}
	\caption{The accuracy of Algorithm \ref{alg1} in four quadrants with different $rv$ and $rf$, where we treat $rv\cdot l$ keywords with highest volume as high-volume keywords and treat $rf\cdot l$ keywords with highest frequency as high-frequency keywords (A larger $rv$ means more queries are considered as high-volume queries. Similarly, a larger $rf$ yields more queries are categorized as high-frequency queries). The three rows show the results on Enron, Lucene, and Wikipedia (in that order), respectively. }
	\label{fig:quadrants_wiki}
\end{figure*}





\begin{figure*}[!t]
	\centering
	
	\subfigure[HVHF]
	{
 \label{HVHF_enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/HVHF.pdf}
		\end{minipage}
	}
	\subfigure[HVLF]
	{
 \label{HVLF_enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/HVLF.pdf}
		\end{minipage}
	}
        \subfigure[LVHF]
	{
 \label{LVHF_enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/LVHF.pdf}
		\end{minipage}
	}
        \subfigure[LVLF]
	{
 \label{LVLF_enron}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/LVLF.pdf}
		\end{minipage}
	}

	
	\subfigure[HVHF]
	{
 \label{HVHF_lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/HVHF.pdf}
		\end{minipage}
	}
	\subfigure[HVLF]
	{
 \label{HVLF_lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/HVLF.pdf}
		\end{minipage}
	}
        \subfigure[LVHF]
	{
 \label{LVHF_lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/LVHF.pdf}
		\end{minipage}
	}
        \subfigure[LVLF]
	{
 \label{LVLF_lucene}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/LVLF.pdf}
		\end{minipage}
	}

	
	\subfigure[HVHF]
	{
 \label{HVHF_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/HVHF.pdf}
		\end{minipage}
	}
	\subfigure[HVLF]
	{
 \label{HVLF_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/HVLF.pdf}
		\end{minipage}
	}
        \subfigure[LVHF]
	{
 \label{LVHF_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/LVHF.pdf}
		\end{minipage}
	}
        \subfigure[LVLF]
	{
 \label{LVLF_Wiki}
		\begin{minipage}{.235\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/LVLF.pdf}
		\end{minipage}
	}
	\caption{The accuracy of Algorithm \ref{alg1} on four quadrants with different $\alpha$, where $\alpha$ is weight of volume and $(1-\alpha)$ is weight of frequency in measurement. The three rows show the results on Enron, Lucene, and Wikipedia (in that order), respectively.
 }
	\label{fig:quadrants_test_alpha}
\end{figure*}
% \begin{figure*}[!t]
% 	\centering
	
% 	\subfigure[HVHF]
% 	{
%  \label{HVHF_enron}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/HVHF.pdf}
% 		\end{minipage}
% 	}
% 	\subfigure[HVLF]
% 	{
%  \label{HVLF_enron}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/HVLF.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[LVHF]
% 	{
%  \label{LVHF_enron}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/LVHF.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[LVLF]
% 	{
%  \label{LVLF_enron}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_enron/LVLF.pdf}
% 		\end{minipage}
% 	}
% 	\caption{The accuracy of Algorithm \ref{alg1} in Enron of four quadrants with different $\alpha$, where $\alpha$ is weight of volume and $(1-\alpha)$ is weight of frequency in measurement.}
% 	\label{fig:quadrants_test_alpha_enron}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
	
% 	\subfigure[HVHF]
% 	{
%  \label{HVHF_lucene}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/HVHF.pdf}
% 		\end{minipage}
% 	}
% 	\subfigure[HVLF]
% 	{
%  \label{HVLF_lucene}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/HVLF.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[LVHF]
% 	{
%  \label{LVHF_lucene}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/LVHF.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[LVLF]
% 	{
%  \label{LVLF_lucene}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_lucene/LVLF.pdf}
% 		\end{minipage}
% 	}
% 	\caption{The accuracy of Algorithm \ref{alg1} in Lucene of four quadrants with $\alpha$, where $\alpha$ is weight of volume and $(1-\alpha)$ is weight of frequency in measurement.}
% 	\label{fig:quadrants_test_alpha_lucene}
% \end{figure*}


% \begin{figure*}[!t]
% 	\centering
	
% 	\subfigure[HVHF]
% 	{
%  \label{HVHF_Wiki}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/HVHF.pdf}
% 		\end{minipage}
% 	}
% 	\subfigure[HVLF]
% 	{
%  \label{HVLF_Wiki}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/HVLF.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[LVHF]
% 	{
%  \label{LVHF_Wiki}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/LVHF.pdf}
% 		\end{minipage}
% 	}
%         \subfigure[LVLF]
% 	{
%  \label{LVLF_Wiki}
% 		\begin{minipage}{.235\linewidth}
% 			\centering
% 			\includegraphics[width=\linewidth]{pic/test_alpha/pic_wiki/LVLF.pdf}
% 		\end{minipage}
% 	}
% 	\caption{The accuracy of Algorithm \ref{alg1} in Wikipedia of four quadrants with $\alpha$, where $\alpha$ is weight of volume and $(1-\alpha)$ is weight of frequency in measurement.}
% 	\label{fig:quadrants_test_alpha_wiki}
% \end{figure*}


==> figures_in_test_beta_with_f.tex <==
\begin{figure*}[!t]
	\centering
	
        
	\subfigure[Enron]
	{
 \label{fig:test_beta_enron}
		\begin{minipage}{.3\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/test_beta/enron_with_freq.pdf}
		\end{minipage}
	}
	\subfigure[Lucene]
	{
 \label{fig:test_beta_lucene}
		\begin{minipage}{.3\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_beta/lucene_with_freq.pdf}
		\end{minipage}
	}
        \subfigure[Wikipedia]
	{
 \label{fig:test_beta_wiki}
		\begin{minipage}{.3\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_beta/wiki_with_freq.pdf}
		\end{minipage}
	}
	\caption{The accuracy of our attack with different $\beta$, where $beta$ is the weight of co-occurrence information and $(1-\beta)$ is the weight of volume and frequency information in calculating $score$.}
	\label{fig:test_beta_with_freq}
\end{figure*}

==> figures_in_test_beta_without_f.tex <==
\begin{figure*}[!t]
	\centering
	\subfigure[Enron]
	{
 \label{fig:test_beta_enron_without_f}
		\begin{minipage}{.3\linewidth}
			\centering
                \includegraphics[width=\linewidth]
                {pic/test_beta/enron_without_freq.pdf}
		\end{minipage}
	}
	\subfigure[Lucene]
	{
 \label{fig:test_beta_lucene_enron_without_f}
		\begin{minipage}{.3\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_beta/lucene_without_freq.pdf}
		\end{minipage}
	}
        \subfigure[Wikipedia]
	{
 \label{fig:test_beta_wiki_enron_without_f}
		\begin{minipage}{.3\linewidth}
			\centering
			\includegraphics[width=\linewidth]{pic/test_beta/wiki_without_freq.pdf}
		\end{minipage}
	}
	\caption{The accuracy of our attack with different $\beta$ without frequency information, where $beta$ is the weight of co-occurrence information and $(1-\beta)$ is the weight of volume and frequency information in calculating $score$.}
	\label{fig:test_beta_without_freq}
\end{figure*}
